A Contraction Theory Approach to Stochastic Incremental Stability

We investigate the incremental stability properties of It\^o stochastic dynamical systems. Specifically, we derive a stochastic version of nonlinear contraction theory that provides a bound on the mean square distance between any two trajectories of a stochastically contracting system. This bound can be expressed as a function of the noise intensity and the contraction rate of the noise-free system. We illustrate these results in the contexts of stochastic nonlinear observers design and stochastic synchronization.

==> synchro.tex <==


%%%LocalVariables:
%%%mode:latex
%%%TeX-master:"stocon"
%%%End:

